cedar: Optimized and Unified Machine Learning Input Data Pipelines

The input data pipeline is an essential component of each machine learning (ML) training job. It is responsible for reading massive amounts of training data, processing batches of samples using complex transformations, and loading them onto training nodes at low latency and high throughput. Performant input data systems are becoming increasingly critical, driven by skyrocketing data volumes and training throughput demands. Unfortunately, current input data systems cannot fully leverage key performance optimizations, resulting in hugely inefficient infrastructures that require significant resources - or worse - underutilize expensive accelerators. To address these demands, we present cedar, an optimized and unified programming framework for ML input data pipelines. cedar allows users to define input data pipelines using composable operators that support arbitrary ML frameworks and libraries. cedar introduces an extensible optimizer that systematically applies a complex combination of optimizations (e.g., offloading, caching, prefetching, fusion, and reordering). It orchestrates processing across a customizable set of local and distributed compute resources in order to improve processing performance and efficiency, all without user input. Across eight pipelines, cedar improves performance by up to 1.87x to 10.65x compared to state-of-the-art input data systems.

==> evaluation_old.tex <==
\section{Evaluation}\label{sec:evaluation}
We designed \systemname to support the numerous libraries and frameworks currently used across ML deployments. %
Since ML practitioners predominantly rely on Python, \systemname is built from the ground up in $\sim$12K lines of Python.
\systemname supports all popular ML frameworks (e.g., PyTorch, JAX, and TensorFlow) and can execute operations from arbitrary preprocessing libraries that provide a Python API. 

\noindent\textbf{Workloads.}
\input{figures/tbl/pipelines_eval}
We evaluated \systemname on a diverse set of six ML input data pipelines across computer vision, natural language, and speech domains as shown in Table~\ref{tbl:pipelines_eval}.
\texttt{CV-torch} is the SimCLR~\cite{arxiv:chen_simclr, arxiv:chen_simclrv2} pipeline in Figure~\ref{fig:simclr}, implemented using torchvision, while \texttt{CV-tf} reimplemented the same operations using native TensorFlow (TF) image~\cite{website:tf.image} operators.
SimCLR is a common vision task requiring compute-intensive operations and thus performant input data systems~\cite{atc22:graur_cachew}.
We used ImageNet~\cite{cvpr09:deng_imagenet} as the dataset for both \texttt{CV} pipelines, and both utilized the exact semantic constraints shown in Figure~\ref{fig:feature_api}.
The \texttt{NLP} pipelines are based on GPT-2~\cite{techreport:radford_gpt2} and represent a typical language pipeline (e.g., for training and fine-tuning LLMs~\cite{arxiv:gpt3}).
\texttt{NLP-torch} was implemented using torchtext with a Byte Pair Encoding (BPE) tokenizer.
\texttt{NLP-hf-tf} implemented the same operations using tf.text~\cite{website:tftext}, but used a Hugging Face BPE tokenizer~\cite{website:huggingface-transformers}.
Finally, \texttt{NLP-tf} used all TF native operators, including a SentencePiece tokenizer from tf.text.
We used the WikiText-103 dataset~\cite{arxiv:merity_wikitext} for all NLP pipelines.
All \texttt{NLP} operators were fixed in location and none were random.
\texttt{ASR} implements SpecAugment~\cite{interspeech19:park_specaugment}, used for speech recognition tasks.
In addition to requiring compute-intensive operations, \texttt{ASR} represents a common case where pipelines use third-party domain-specific libraries.
\texttt{ASR} was implemented using librosa~\cite{scipy15:mcfee_librosa}, and it used the Common Voice dataset~\cite{arxiv:ardila_commonvoice}.
All \texttt{ASR} operators were fixed except for Stretch, TimeMask, and FreqMask.
TimeMask and FreqMask were random. 


\subsection{Combining Optimization Techniques}
We begin by evaluating how effective \systemname's ability to combine optimizations is at improving performance compared to state-of-the-art input data systems.
Specifically, to isolate the efficacy of \systemname's static optimizations, we first focus on the same metric as in Section~\ref{sec:optimizations_space} -- the time needed to process a given amount of samples using a fixed set of resources, with unbounded training demand (i.e., as fast as possible).
Systems with a lower execution time -- higher throughput -- using the same set of resources can both better eliminate data stalls and achieve higher efficiency given a training throughput demand.
This is because an effective auto-tuner (which we evaluate in Section~\ref{sec:eval_autotune}) can use fewer resources to meet demand.




\noindent\textbf{Can \systemname optimize the performance of local input data processing?}
Since training nodes often offer a large amount of CPU host resources~\cite{website:dgxh100}, %
we first compared \systemname against four state-of-the-art input data frameworks, all performing processing on a single VM (n2-standard-8 on Google Cloud).
\texttt{tf} used TensorFlow's tf.data~\cite{vldb14:murray_tfdata}, and we allowed tf.data to optimize the parallelism of each operator.
\texttt{plumber}~\cite{mlsys22:kuchnik_plumber} extended tf.data to use a linear program to allocate resources across operators.
\texttt{ray-local} used the Ray Data framework which executed input data processing using Arrow~\cite{website:arrow} on top of Ray~\cite{website:ray-data}.
\texttt{torch} used the PyTorch DataLoader~\cite{website:torch-utilsdata}, configured with 8 workers (one per CPU core).


We compared these systems against \texttt{cedar-local} using a single \texttt{Client}; we allowed \texttt{cedar-local} to launch multiple \texttt{Drivers}, and we disabled caching.
We provided \texttt{cedar-local} with a Python multiprocessing engine.
To demonstrate the benefits of \systemname's ability to \textit{choose} to use diverse engines, we also provided \systemname with two engines that can execute operators using tf.data or Ray Data, respectively.
Datasets were stored on the VM's file system.
Figure~\ref{fig:local_eval} shows the execution time to process the dataset, normalized to the \texttt{cedar-local} result for each pipeline (lower is better).
Red X's denote the how \textit{specialized} frameworks cannot support all pipelines.

\input{figures/tex/local_eval}

For the \texttt{CV} pipelines, \systemname was able to reduce execution time (i.e., improve throughput) compared to baselines because it reordered size-reducing operators (crop, grayscale) towards the beginning of the pipeline and size-increasing operators (float) towards the end of the pipeline.
This significantly reduced work for each sample while obeying dependency constraints (crop $\rightarrow$ flip, float $\rightarrow$ normalize).
\systemname also leveraged local parallelism by using 8 \texttt{Drivers}.
\texttt{tf} achieved a similar performance due to its graph optimizer and performant C++ backend.
While \texttt{plumber} was also able to use these TensorFlow benefits, its LP under-allocated parallelism to the decode operator, causing an I/O bottleneck reading images from disk.

For \texttt{NLP-torch} and \texttt{NLP-hf-tf}, \systemname fused Read, Tokenize, and Truncate into one \texttt{Pipe}, which it offloaded to the multiprocess engine.
Meanwhile, \systemname spawned only one \texttt{Driver} within the main \texttt{Client} process.
This avoided a significant serialization bottleneck in sending large embeddings between processes which hampered \texttt{torch} and \texttt{ray-local} on \texttt{NLP-torch}.
For \texttt{NLP-hf-tf}, \systemname out-performed \texttt{tf} because \texttt{tf} could not optimize the non-native Tokenizer operator.
\systemname achieved a slightly lower throughput ($0.85\times$) to \texttt{ray-local}, as its Arrow core allowed it to zero-copy intermediate NumPy arrays. %
\systemname's extensibility allows it to adopt Arrow as a future \texttt{Variant}.
For \texttt{NLP-tf}, \texttt{tf} was able to compile the pipeline into a heavily-optimized TF graph.
In fact, \systemname recognized the performance benefit and offloaded execution to tf.data, \textit{without requiring users to change the \texttt{Feature}}, allowing \systemname to near \texttt{tf}'s throughput ($0.91\times$ due to tracing overheads) and out-perform \texttt{ray-local}. %
\texttt{plumber} could not support any of the NLP pipelines, as it does not support non-native operators or operators that require non-serializable assets (i.e., the tokenizer model).

For \texttt{ASR}, \systemname first pushed Stretch later (to decrease sample sizes) and then offloaded execution to the Ray Data engine, obtaining its zero-copy benefits and matching \texttt{ray-local}'s performance.
Meanwhile, \texttt{torch} and \texttt{tf} suffered from copy overheads.
Because TensorFlow could not trace the pipeline as a graph, \texttt{tf} was forced to execute all operators within its GIL-bound Python process, and \texttt{plumber} could not execute \texttt{ASR} for the aforementioned reasons.

These results highlight the impact of \systemname's extensible optimizer -- optimizing the dataflow via reordering and fusion, offloading and prefetching execution to the best engine, and supporting a diverse set of pipelines -- all without user input.
This allows \systemname to out-perform tf.data, Plumber, Ray Data, and PyTorch DataLoaders by $2.49\times$, $1.30\times$, $2.18\times$, and $2.74\times$ on average, respectively.




\input{figures/tex/remote_eval}
\noindent\textbf{Can \systemname optimize distributed input data processing?}
We next compared \systemname to three baselines that support distributed processing, providing each a remote 32-core VM (n2-standard-32) in addition to the 8-core local VM.
\texttt{tf-service} used tf.data service~\cite{socc23:audibert_tfdataservice} to execute processing on the remote VM; as with \texttt{tf}, we enabled its underlying optimizations. %
\texttt{fastflow}~\cite{vldb16:um_fastflow} extended tf.data service, splitting processing between the local and remote VM.
\texttt{ray-remote} created a Ray cluster across both VMs and used Ray Data.
In addition to the local engines above, we provided \texttt{cedar-remote} with a \texttt{distributed} engine that executes processing remotely using Ray~\cite{osdi18:moritz_ray} tasks.
To standardize data reading, we allowed each system to read raw data from either the local or remote VM's file system. 
\texttt{tf-service} read from the remote VM since all operators were executed remotely.
\texttt{ray-remote} and \texttt{fastflow} spawned tasks on both VMs; each task read from its respective file system.
Meanwhile, \texttt{cedar-remote} selectively offloaded reading, depending on the ideal plan for each pipeline.
As before, we disabled caching. %

Figure~\ref{fig:remote_eval} shows the normalized execution time (lower is better) for each pipeline. %
Because \texttt{tf-service} and \texttt{fastflow} distribute TF graphs to remote workers, they are unable to support non-native pipelines that cannot be traced.
For the \texttt{CV} pipelines, \systemname generated a similar reordering to \texttt{cedar-local} and used 8 \texttt{Drivers}.
It also offloaded the entirety of the pipeline to the distributed engine, \textit{except} for the float conversion and normalization.
Doing so reduced the I/O to a quarter (int8 versus float32) compared to offloading the entire pipeline. %
In contrast, \texttt{ray-remote} did not optimize for I/O (not selectively offloading operators) nor compute costs (not reordering) for both pipelines.
For \texttt{CV-tf}, TensorFlow's graph optimizations allowed \texttt{tf-service} to match \systemname. %
Meanwhile, \texttt{fastflow} achieved slower performance due to resource contention on the local VM between I/O from the remote worker and local processing.

For \texttt{NLP-torch} and \texttt{NLP-hf-tf}, \systemname offloaded the Read, Tokenize, and Truncate operators to a fused distributed \texttt{Pipe}.
As with \texttt{cedar-local}, \systemname performed the embedding operator in the single-\texttt{Driver Client}, avoiding serialization overheads.
Interestingly, \systemname correctly identified that \textit{not} using the remote VM was the optimal plan for \texttt{NLP-tf}; it instead offloaded processing to the \textit{local} tf.data engine. %
Meanwhile, \texttt{tf-service} \textit{did} distribute processing and was bottlenecked by reading large embeddings over the network.
\texttt{fastflow} was able to intelligently execute processing locally, but incurred significant overheads as it inserted additional logic that limited the benefit of TensorFlow's graph compiler.
\systemname outperformed \texttt{ray-remote} across \texttt{NLP} because \texttt{ray-remote} not only inefficiently read large embeddings over RPCs, but it also held embeddings within its object store, quickly saturating it and causing frequent spills to disk.
Finally, \systemname automatically determined that reordering and offloading \texttt{ASR} to a Ray Data engine (distributed across both VMs) was ideal for the same zero-copy benefits as \texttt{cedar-local}, allowing it to match \texttt{ray-remote}.

\systemname is able to effectively apply its optimizations to distributed processing.
On average, \systemname outperformed \texttt{ray-remote}, \texttt{fastflow}, and \texttt{tf-service} by $2.19\times$, $2.35\times$, and $1.87\times$, respectively.


\input{figures/tbl/autotune_static_eval}
\input{figures/tbl/autotune_eval}
\subsection{Auto-tuning Parallelism}\label{sec:eval_autotune}
\noindent\textbf{Can \systemname dynamically right-size resources?}
While \systemname's \texttt{Optimizer} is effective at maximizing raw throughput on a per-resource basis, its \texttt{Auto-Tuner} is responsible for correctly right-sizing the amount of resources used to meet a given throughput demand, thereby maximizing efficiency. %
To evaluate this, we used the \texttt{cedar-remote} scenario with the \texttt{CV-torch} pipeline (other pipelines show similar results but are omitted due to space).
Table~\ref{tbl:autotune_static_eval} shows the throughput achieved by a \texttt{Driver} given a fixed scale (number of remote processes) on the \texttt{distributed} engine, which \texttt{cedar-remote} used to execute the fused operator as mentioned above. %
An effective auto-tuner needs to select the minimal number of processes that achieves a higher throughput than demanded.

Thus, we simulated a training job by requesting samples at fixed rates, as shown in the left column of Table~\ref{tbl:autotune_eval}.
We then configured \systemname to begin with 1 \texttt{distributed} process and allowed \systemname to tune its scale; the right column reports the steady-state tuned number of processes.
First, \systemname is effective at minimizing the number of processes needed to meet a requested throughput, without under-provisioning resources.
Secondly, \systemname's ability to \textit{dynamically} mutate a \texttt{Pipe}'s \texttt{Variant} can even completely free the remote VM in the case of low training throughput, in contrast to systems such as tf.data service~\cite{socc23:audibert_tfdataservice} and Cachew~\cite{atc22:graur_cachew} which \textit{always} use distributed processing.
These results show that \systemname is able to translate the high performance provided by its \texttt{Optimizer} to high resource efficiency to meet a throughput demand.



\subsection{Understanding Optimizations}\label{sec:eval_ablation}
Finally, we explore in-depth the importance of combining multiple optimizations, and we evaluate \systemname's ability to apply caching.

\noindent\textbf{How do each of \systemname's optimizations contribute to performance?} 
\input{figures/tex/ablation_eval}
To understand \systemname's ability to \textit{combine} optimizations, we performed an ablation study by successively enabling local parallelism (i.e., multiple \texttt{Drivers}), reordering, offloading (enabling the \texttt{distributed} engine), and fusion.
All experiments used prefetching.
Figure~\ref{fig:ablation_eval} shows the execution time of each experiment, normalized to the baseline (i.e., executing the unoptimized \texttt{DataSet} within a single \texttt{Driver}).
No single optimization is a panacea. %
Instead, a diverse set of optimizations is needed to achieve high performance due to the diverse characteristics across pipelines.

Local parallelism was effective for \texttt{CV-torch} and \texttt{ASR} since using multiple \texttt{Drivers} bypassed their GIL bottleneck.
\texttt{CV-tf} largely used multithreaded C++ operators, limiting this benefit. %
\systemname did not parallelize the NLP pipelines to avoid serialization overheads.
Reordering was effective at improving both \texttt{CV} pipelines since they used size-changing operators. %
Meanwhile, \texttt{ASR} had more limited reordering opportunities, and the \texttt{NLP} pipelines were not able to be reordered.
All pipelines ultimately took advantage of offloading across engines.
However, the overheads incurred by data movement across offloaded pipes limited its effectiveness for some pipelines.
By eliminating these overheads with fusion, \systemname was ultimately able to improve throughput by $2.54-43.82\times$ compared to the baseline.
The successive improvements with each step showcase \systemname's ability to systematically apply and combine optimizations. 


\input{figures/tbl/caching_eval}
\noindent\textbf{Can \systemname automatically cache to maximize throughput?}
We also evaluated if \systemname can reason about \textit{if} and \textit{where} caching would be beneficial.
To do so, we allowed \systemname to automatically place a Cache \texttt{Pipe}, which materialized all intermediate samples to disk in the first epoch.
We then ran multiple epochs of the torch pipelines across the three domains (\texttt{CV-torch}, \texttt{NLP-torch}, and \texttt{ASR}).
Table~\ref{tbl:caching_eval} shows the throughput (higher is better) of the cached plan after the first epoch, normalized to the throughput achieved by the plan generated by \texttt{cedar-remote}.
We also report the \textit{next-best} throughput achieved by enumerating all other cache locations.
\systemname was able to find the optimal location to apply caching.

For \texttt{CV-torch}, \systemname cached the result after decode and grayscale, but prior to random cropping, satisfying randomness requirements.
This improved throughput by reducing disk I/O (decode) and compute (grayscale).
For \texttt{NLP-torch}, \systemname cached the tokenized and truncated sample \textit{prior} to embedding, avoiding overheads of reading large embeddings.
Interestingly, \systemname did \textit{not} cache \texttt{ASR}, determining that re-computation was ideal because transforms significantly increased data volumes.
Table~\ref{tbl:caching_eval} confirms this; the next ``best'' solution cached the output of the entire pipeline, which \textit{reduced} throughput by $18\%$.
\systemname is effectively able to apply caching while reasoning about its complex interactions with other optimizations. 

==> figures/tbl/autotune_eval.tex <==
\begin{table}[t]
\centering
\caption{Number of processes tuned to by the \texttt{Auto-Tuner} to reach a target training throughput (samples/s) for \texttt{CV-torch}.}\label{tbl:autotune_eval}
\small
\begin{tabular}{@{}l|l@{}} \toprule
Required GPU Rate & Auto-Tuned \# Processes \\ \midrule
39.83        & 0 [Used \textit{base} \texttt{Variant}]                  \\ %
194.40       & 4                     \\ %
379.13     & 8                     \\ %
559.11     & 12   \\ \bottomrule                
\end{tabular}
\end{table}

==> figures/tbl/autotune_static_eval.tex <==
\begin{table}[t]
\centering
\caption{Steady-state throughput (samples/s) for a static number of offloaded processes for the \texttt{CV-torch} pipeline.}\label{tbl:autotune_static_eval}
\small
\begin{tabular}{@{}l|lllll@{}}
\toprule
           & Local   & 1 Proc.   & 2 Procs. & 4 Procs.  & 8 Procs.   \\ \midrule
Samples/s & 70.77 & 71.43 & 128.61 & 245.11 & 438.91 \\ \bottomrule
\end{tabular}
\end{table}

==> figures/tex/local_eval.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[width=\linewidth]{figures/img/local.png} 
  \caption{Execution time (lower is better) for local systems across six pipelines, normalized to \texttt{cedar-local} for each. Red X's denote incompatible frameworks.}
  \label{fig:local_eval}
\end{figure}


==> figures/tex/remote_eval.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[width=\linewidth]{figures/img/remote.png} 
  \caption{Execution time (lower is better) for distributed systems across six pipelines, normalized to \texttt{cedar-remote} for each. Red X's denote incompatible frameworks.}
  \label{fig:remote_eval}
\end{figure}

